Enabling Cost-Effective Blockchain Applications via Workload-Adaptive Transaction Execution

As transaction fees skyrocket today, blockchains become increasingly expensive, hurting their adoption in broader applications. This work tackles the saving of transaction fees for economic blockchain applications. The key insight is that other than the existing "default" mode to execute application logic fully on-chain, i.e., in smart contracts, and in fine granularity, i.e., user request per transaction, there are alternative execution modes with advantages in cost-effectiveness. On Ethereum, we propose a holistic middleware platform supporting flexible and secure transaction executions, including off-chain states and batching of user requests. Furthermore, we propose control-plane schemes to adapt the execution mode to the current workload for optimal runtime cost. We present a case study on the institutional accounts (e.g., coinbase.com) intensively sending Ether on Ethereum blockchains. By collecting real-life transactions, we construct workload benchmarks and show that our work saves 18% ~ 47% per invocation than the default baseline while introducing 1.81 ~ 16.59 blocks delay.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sty/common-newdefines.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}

%obsoleted due to reviewer complains definition without number
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}




==> sty/ieeetran/ieee-template/editable/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/ieee-template/inputs/README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> sty/ieeetran/titlepage.tex <==
\input{sty/title.tex}
\author{
\ifdefined\TTUT
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\fi
}

\maketitle
\IEEEpeerreviewmaketitle



==> sty/ieeetran/usepackage.tex <==
%using latex.XXX file to cusotmize style
%\usepackage{./sty/ieeetran/latex}



==> sty/llncs2e/titlepage.tex <==
\input{sty/title.tex}
\author{
Kai Li\hspace{0.25cm}
Yuzhe (Richard) Tang\hspace{0.25cm}
Beom Heyn (Ben) Kim$\ ^\dag{}$\hspace{0.25cm}
Jianliang Xu$\ ^\ddag{}$\hspace{0.25cm}\\
\ifdefined\TTUT
\fi
}

\institute{
    \fontsize{10}{10}\selectfont\itshape
    Syracuse University, New York, USA\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag{}$University of Toroto, Ontario, Canada\\
    \fontsize{10}{10}\selectfont\itshape
    $^\ddag{}$Hong Kong Baptist University, Kowloon Tong, Hong Kong 
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/titlepage.tex <==
\input{sty/title.tex}
\author{
Yuzhe Tang$\ ^\dag$\hspace{1cm}Author2$\ ^\ddag$\hspace{1cm}Author3$\ ^\S$\hspace{1cm}Author4$\ ^\sharp$\\
    \fontsize{10}{10}\selectfont\itshape
    $^\dag$Syracuse University, NY, USA, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    ytang100@syr.edu\\
    \fontsize{10}{10}\selectfont\rmfamily\itshape
    $^\ddag$Hong Kong Baptist University, Kowloon Tong, Hong Kong,
    Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    author2@affiliation.edu\\
    \fontsize{10}{10}\selectfont\itshape
    $^\S{} ^\sharp{}$Fudan University, Shanghai, China, Email:
    \fontsize{9}{9}\selectfont\ttfamily\upshape
    \{author3, author4\}@affiliation.edu
\ifdefined\TTUT
\fi
}

\maketitle



==> sty/report/usepackage.tex <==
\usepackage{etoolbox}
\makeatletter
\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
\makeatother

\usepackage{titlesec}
{\filcenter\normalfont\Large\bfseries}
\titleformat{\chapter}
  {\normalfont\sffamily\LARGE\it}
  {\thechapter.}{10pt}{\LARGE}
\titlespacing*{\chapter}{0pt}{0pt}{0pt}
\titleformat{\section}
  {\normalfont\sffamily\Large\bfseries}
  {\thesection.}{0.3em}{}
\titleformat{\subsection}
  {\normalfont\sffamily\large\it}
  {\thesubsection.}{0.3em}{}





==> sty/sig-alternate/titlepage.tex <==
\input{sty/title.tex}
\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\numberofauthors{4} % if number of authors is bigger than number of \alighauthor used following, a ``addtional author'' section will be shown in the end of the paper.
%note: no empty line!
\author{
\alignauthor
Yuzhe Tang$^\dag$
%\titlenote{Author notes}
\\       \affaddr{Syracuse University}
\\       \affaddr{Syracuse, NY 13244}
\\       \email{$^\dag$ytang100@syr.edu}
\ifdefined\TTUT
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\and
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
% 2nd. author
\alignauthor
Yuzhe Tang\titlenote{Author notes}\\
       \affaddr{Syracuse University}\\
       \affaddr{Syracuse, NY 13244}\\
       \email{ytang100@syr.edu}
\fi
}
\date{30 July 1999}
\maketitle



==> sty/sig-alternate/titlepage_sharedAuthorAddr.tex <==
\begin{document}
%
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
%
\linespread{0.9}

% --- Author Metadata here ---
\conferenceinfo{WWW}{'13 Rio de Janerio, Brazil}
\title{
Tang's Template of IEEEtran.cls for Conferences \titlenote{!Eye-catching title for high citation: make it short}
}

\subtitle{[Extended Abstract] \titlenote{full version is available at \texttt{www.acm.org/eaddress.htm}}}

\numberofauthors{1}
\author{
\alignauthor Yuzhe Tang, Ting Wang and Ling Liu \\
  \affaddr{College of Computing, Georgia Institute of Technology} \\ 
  \affaddr{ Atlanta, GA 30332, USA} \\
  \email{yztang@gatech.edu, \{twang, lingliu\}@cc.gatech.edu}
}
\date{30 July 1999}
\maketitle



==> sty/title.tex <==
\begin{document}
% --- Author Metadata here ---
\title{\Huge Efficiently Hardening SGX Enclaves against Memory Access Pattern Attacks via Dynamic Program Partitioning}



==> sty/usenix/titlepage.tex <==
\input{sty/title.tex}

\ifdefined\TTUT
\author{
{\rm Your N.\ Here}\\
Your Institution
\and
{\rm Second Name}\\
Second Institution
% copy the following lines to add more authors
% \and
% {\rm Name}\\
%Name Institution
} % end author
\fi

\maketitle

% Use the following at camera-ready time to suppress page numbers.
% Comment it out when you first submit the paper for review.
\thispagestyle{empty}





==> sty/usenix/usepackage.tex <==
\usepackage{sty/usenix/usenix,epsfig,endnotes}


==> sty/usepackage_config2.tex <==
%using latex.XXX file to cusotmize style
%customized tools
\let\Bbbk\relax
\usepackage{amssymb}
\usepackage{times}
\usepackage{amsfonts}
%\usepackage{amsthm}

\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{float}
\usepackage{multirow, graphicx}
\usepackage{algorithm}
\usepackage{algpseudocode} %algorithm: use algorithmicx package, to refer to http://en.wikibooks.org/wiki/LaTeX/Algorithms_and_Pseudocode#Typesetting_using_the_algorithmicx_package
\usepackage{amsmath}

%squeeze space 
\setlength{\belowcaptionskip}{2pt}
\setlength{\abovecaptionskip}{2pt}
\setlength{\floatsep}{0.25\floatsep}
\setlength{\dblfloatsep}{0.25\dblfloatsep}
\setlength{\textfloatsep}{0.25 \textfloatsep}
\setlength{\dbltextfloatsep}{0.25\dbltextfloatsep}
\setlength{\intextsep}{0.25\intextsep}

%reduce whitespace surrounding section titles.
%\newcommand{\subparagraph}{} %from stackexchange: The titlesec package assumes all of the section levels provided by the standard classes are present. This includes the subparagraph level. The IEEEtrans class doesn't define a level subparagraph
%\usepackage[compact]{titlesec}  
%\titleformat{\paragraph}[runin]{\normalfont\itshape}{\theparagraph}{3pt}{} %keep paragraph title in the same line.
%TODO: to add manually a ":" to each of paragraph headings!

%TODO: to manually add \vspace{-.5cm} into authors and paper title, which reduce the whitespace in the front page.

%\usepackage{sty/simplemargins}
%    \setleftmargin{0.6in}
%    \setrightmargin{0.70in}
%    \settopmargin{0.55in}
%    \setbottommargin{0.55in}

%use to set line spacing for whole document
%f:http://en.wikibooks.org/wiki/LaTeX/Paragraph_Formatting#Line_spacing
%\usepackage{setspace} %dont use this alone (with sig-alternate)! footnote with 9 will show.
%\singlespacing
%\onehalfspacing
%\doublespacing
%\setstretch{1.1}


\usepackage{xspace}

%url
\usepackage{url}
\def\UrlBreaks{\do\/\do-}
%%\usepackage[breaklinks]{hyperref}
\usepackage{breakurl}

\usepackage{sty/widetext} %show equation in two columns

\usepackage{stackrel}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

%cut words in middle when running out of space in a line.

%\pagestyle{empty} %this removes the page number
%\pagenumbering{gobble} %this really remove page numbers
\thispagestyle{plain}
\pagestyle{plain} %this enforce page number

\ifdefined\TTSTYLETARGETreport
% bibliography
\usepackage[
    backend=bibtex,
    maxbibnames=100,
    firstinits=true,
    bibstyle=numeric,
    citestyle=numeric
%    bibstyle=alphabetic,
%    citestyle=alphabetic
]{biblatex}
\addbibresource{ads.bib}
\addbibresource{lsm.bib}
\addbibresource{bkc.bib}
\addbibresource{dos.bib}
\addbibresource{odb.bib}
\addbibresource{cacheattacks.bib}
\addbibresource{sc.bib}
\addbibresource{crypto.bib}
\addbibresource{sgx.bib}
\addbibresource{diffpriv.bib}
\addbibresource{txtbk.bib}
\addbibresource{distrkvs.bib}
\addbibresource{vc.bib}
\addbibresource{yuzhetang.bib}
\fi

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

%todonotes
\usepackage{todonotes}
\newcommand{\tangSide}[1]{\todo[caption={},color=cyan!20!]{{\tiny Note: #1}}}
\setlength{\marginparwidth}{1.5cm}
\newcommand{\ignore}[1]{}

\input{sty/wheels-usepackage.tex}
\sloppy


==> text/V1_paper.tex <==
\section{Introduction}

The Ethereum blockchain~\cite{me:eth2} is the second largest blockchain after Bitcoin and the largest blockchain that supports smart contracts. The Ethereum blockchain is rapidly gaining popularity. Ethereum charges a very high fee for transaction execution. The data storage and processing of a transaction are expensive because of the distributed structure of blockchain. Due to the intensive use with capacity constraints, the Ethereum users compete the	price with each other to make their transactions included in the blockchain. The price of Ether has increased $27$ times in $2$ years (at the exchange rate as of Mar. 2022). The high transaction fee has discouraged the Ethereum users and finally shrinks the Ethereum ecosystem.

There are several cost saving schemes on blockchain that have been studied in the existing literature. iBatch~\cite{DBLP:conf/sigsoft/WangZLTCLC21} supports batching multiple smart-contract invocations into one transaction so that the base fee is amortized. GruB~\cite{DBLP:conf/middleware/LiTCYXX20} stores data off-chain in write-intensive workloads and dynamically replicates the data on the blockchain. Layer-two protocols~\cite{me:lightning,DBLP:journals/corr/MillerBKM17,DBLP:journals/corr/abs-1804-05141,DBLP:conf/ccs/DziembowskiFH18} are built on top of the blockchain. They process the application logic off-chain to increase throughput and reduce gas fee of the transactions between institutional accounts. The comparison of these scheme choices is illustrated in table~\ref{tab:optimization_schemes}. iBatch supports batching smart contract invocations between any kinds of accounts, while it is limited as it doesn’t support Ether transferring. GRuB stores the data off-chain. It is designed only for data-feed workloads and doesn’t support Ether transfer as well. Layer-two protocols support Ether transferring with the payment network. It saves Gas cost only for the transactions between two institutional accounts. 

While iBatch is under smart contract workloads and GruB is under data feed workloads, it remains an open research problem: whether one can optimize the cost of institutional-client sent Ether-transferring transactions without additional trust assumption by leveraging batch and off-chain states?

We tackle this problem by presenting OCIA, a blockchain optimization scheme for institutional accounts via selective off-chain states. OCIA is a control-plane scheme that maps the upper-layer transaction workloads (Ether transfers) to the underlying data plane that extends blockchains with batch transactions (i.e., iBatch) and off-chain states (i.e., GRuB). This work extends the workload to new, more common workloads, that is, Ether transfers from institutional accounts to average accounts. 

We propose a novel mapping scheme that places write-intensive accounts off-chain and read-intensive accounts on-chain. Two execution modes respectively support the transactions sent from on-chain accounts to off-chain accounts and the transactions sent from off-chain accounts to on-chain accounts.

We further propose an (offline) dynamic optimization algorithm that decides when to upload the off-chain states to the on-chain storage (i.e., to convert an off-chain account to on-chain one) in order to maximize the batch size and minimize the cost.

We discover the institutional accounts who send the most transactions in one day Ethereum transaction history. We then analyze 3 institutional accounts’ transaction history as case study workloads including Coinbase, Ethermine, Crypto.com. Without additional delay, the result shows OCIA costs $9.8\%\sim{}42.6\%$ more per invocation than baseline.


\begin{table*}[!htbp] %force in current page, disable float.
  \caption{Cost Optimization Schemes}
  \label{tab:optimization_schemes}
  \centering{\small
  \begin{tabularx}{1.00\textwidth}{ |X|l|l|l|l| }
    \hline 
    Scheme & \multicolumn{2}{l|}{Workload} & Approach & Supported pattern \\ \cline{2-3}
    & Supported & Ether transfer &  &  \\ \hline
  iBatch & Smart Contract & \xmark & Batch requests & \makecell[l]{Any-any \\Institutional-any }   \\ \hline
  GruB & Smart Contract (Data Feed)  & \xmark & Off-chain storage & N/A  \\ \hline
  Layer-2 & Ether Transfer & \cmark & Payment networks & \makecell[l]{Institutional - \\institutional}  \\ \hline
  OCIA & Ether Transfer & \cmark & Batch + Off-chain storage & Institutional - avg \\ \hline
  \end{tabularx}}
  \end{table*}
  

\section{Preliminary: Ethereum transaction model}

In Ethereum, there are two types of blockchain accounts, externally owned account (or EOA) and smart contract account (CA). An account is associated with certain on-chain ``states’’. In the case of EOA, the state is the account balance. In the case of CA, the state additionally includes the storage variables in the smart contract. 

Each transaction contains multiple instructions and each instruction has a specific cost that is counted in Gas. The transaction sender pays the fee based on the amount of Gas to compensate for the computational effort made by the Ethereum network. Each transaction has a base fee that is $21000$ Gas covering the cost of verifying the signature of the sender as well as uploading the transaction data.

\section{Execution Modes and Cost}
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/system_pull-push3.eps}
  \caption{Execution Modes}
  \label{fig:execution_modes}
  \end{wrapfigure}
Blockchain transactions can be executed in different equivalent modes. By default, account states are on-chain and each client request is executed in a dedicated transaction. Alternatively, states can be placed off-chain, and multiple requests can be batched in transaction. Figure~\ref{fig:execution_modes} shows different execution modes in M1, M2, and M3. Note that we discard the conceptual model dealing with non-batch transaction and on-chain state, because this model does not save costs in our analysis.

In the following, we present M1, M2, and M3 in more details. 

\subsection{Mode M1 (non-batch transactions, on-chain state)}
All accounts’ states are stored on the blockchain (including EOA’s balance and CA’s program data). An EOA’s request to transfer Ether is executed in a dedicated transaction.

To establish the cost model, we consider an over-simplified workload named W1’. In W1’, an institutional account A0 sends a sequence of $N$ Ether-transferring transactions in $L$ blocks. We will consider more generic cases of transactions with multiple senders and smart contracts. Under the simple workload (W1’), the cost under the mode M1 is $21000 * N$, where $21000$ is the cost of sending an Ether-transferring transaction on Ganache v2.4.0/Solidity 0.4.24. Thus, the per-transfer cost is

$C_1 = 21000$

\subsection{Mode M2 (batch transactions, on-chain states)}

In $M2$, accounts’ states are stored on the blockchain. The EOA’s request is batched with other requests, submitted at similar time, in a large transaction. As shown in Figure~\ref{fig:execution_modes}, the batch transaction is sent to a smart-contract, called Dispatcher, that dispatches the individual EOAs’ requests to their corresponding on-chain states. 

iBatch~\cite{DBLP:conf/sigsoft/WangZLTCLC21} materializes M2 with an untrusted Batcher service with resilience to various forms of request manipulation (e.g., replay attacks). Specifically, iBatch’s Dispatcher smart contract verifies the signatures of each batched request and check a transaction-wise nonce. For detailed security analysis against request replay attacks, refer to the paper~\cite{DBLP:conf/sigsoft/WangZLTCLC21}.

Under the workload $W1’(N, L)$, the cost with $M2$ is $21000*L + NW [16 * (20+32) + 7500]$, where 16* (20+32) is the transaction cost storing data field\footnote{$16$ is Gas cost per byte in the data field and the first/second 32 respectively refer to the number of bytes storing the value and receiver address in an Ether transfer.} and 7500 is the cost of calling an internal Ether transfer. Thus, the per-transfer cost is

$C_2 = 21000 L/NW + 8332$

\subsection{Mode M3 (batch transactions, off-chain states)}
Accounts’ states are stored off the blockchain, and clients’ requests are batched in transactions. 

{\bf Sender/receiver off-chain}: The system is built on top of iBatch by placing the account states to an off-chain service. When a request, say Alice transferring Ether to Bob, is batched in a transaction, the on-chain smart contract needs to authenticate Alice’s old balance and update it, to authenticate Bob’s old balance and update it, and compute the digest including Alice’s and Bob’s updated balances before updating the digest on storage. In this process, the transaction’s data will include the Merkle proofs authenticating Alice’s and Bob’s old balances against the old digest. Note that given multiple transfer requests per batch, each transfer’s data (sender, value and receiver) needs to be sent to the blockchain. 

{\bf Sender on-chain, receiver off-chain}: 

\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/system_pull-push42.eps}
  \caption{Sender on-chain receiver off-chain Modes}
  \label{fig:system_m4}
  \end{wrapfigure}
The M3 places the receivers’ states to an off-chain server and the state updating information in a Hash log by expanding the Merkle tree instead of updating the state in off-chain directly. When receiving requests, say A0 transferring Ether to A1 and A2, we add delta A1 and delta A2 as new leaf nodes and keep the original balance unchanged. In each block, we upload the new digest and the state updating information on-chain, specifically the receiver's addresses and the transfer values. The on-chain smart contract leverages the updating information and the old digest to authenticate the new digest and update the digest on chain. Under workload W1’, the cost is $21000L + NW [16 * (20 + 36) + 222] + (16 * 32 + 5000)L$ where $222$ is the cost of SHA3 Keccak-256 operation of two 32 bytes digest, $16 * 32$ is the cost of uploading the new digest in the call data field and $5000$ is the cost of updating the digest for each block in the on-chain smart contract. Thus, the per-transfer cost is
$C_3 = 26512L/NW + 1118$

\section{Workload Analysis (W1)}

The target workload pattern we optimize is an institutional account $A_0$ sending an intensive stream of requests to other accounts, $A_i$ for $\forall{i\leq{1}}$. As shown in Figure~\ref{fig:system_workload}, given an institutional account $A_0$, there are three transactions of interest in our workload: the transactions sent by $A_0$, the transactions received by $A_i$, and the transactions sent by $A_i$. Here, $A_i$ is an account who receives at least one transaction sent from $A_0$. 

{\bf M1’s costs under workload W1}: For M1, the on-chain states of $A_i$ are updated in Tx1. Hence, the cost of Tx2 is the same as a normal Ether transferring transaction, which is $21000$. Thus, the cost of W1 is 

$C_1 = 21000 * (NW + NR)$

{\bf M2’s costs under workload W1}: For M2, the on-chain states of $A_i$ are updated in Tx1. Hence, the cost of Tx2 is the same as a normal Ether transferring transaction, which is $21000$. Thus, the cost of W1 is 

$C_2 = 21000*L + 8332 * NW + 21000 * NR$

{\bf M3’s costs}: When $A_i$ under M3 transfers Ether to another account, the off-chain server push all the $A_i$ related states on-chain, includes the balance state and the updating value in every blocks. The off-chain server also uploads the Merkle proofs of each updating value and balance state. The on-chain smart contract leverages the Merkle proofs to authenticate the updated balance of $A_i$.  Under workload W1’, say $A_i$ has a initial balance in off-chain server and $A_i$ receive $V_i$ Ether in L blocks, then $A_i$ sends Ether to another account, the cost is $21000L + NR [16 * (20 + 36 + 65) + 6600 + 7500] + NR*16 *(20+L)* 32*L +NR*(20+L)*222+ 5000L$ where $16 * (20 + 36 + 65)$ is the cost of uploading the receiver address, transfer value and sender’s signature, $6600$ is the cost of the verification process of the signature and $7500$ is the cost of an internal Ether transfer. $16 *(20+L)* 32*L$ is the cost of uploading the 20+L-level Merkle proof for L blocks. $(20+L)*222$ is the cost of 20+L SHA3 Keccak-256 operation to verify the digest. 

$C_3 = 26512L + 1118 * NW+ 16036 * NR + NR*16 *(20+L)* 32*L +NR*(20+L)*222$
\begin{wrapfigure}{r}{0.35\textwidth}
  \centering
  \includegraphics[width=0.324\textwidth]{figures/system_workload.eps}
  \caption{System Workload}
  \label{fig:system_workload}
  \end{wrapfigure}

\section{Workload Collection and Results}

\subsection{Discover Institutional Account}

We download the Ethereum Ether transferring transaction and find the Top senders who send most Ether transferring transactions as the institutional accounts on March 1st, 2022. We list the top 10 senders who send most transactions in Table~\ref{tab:institutional-senders}. We then analyze Coinbase, Crypto.com and Ethermine as study cases. We collect the transaction history that was sent from an institutional sender, say A0, to its receivers, say $A_i$. We also get the transactions of Ether transfer that send from $A_i$ after they receive the Ether from A0.
\subsection{The Case of Coinbase}

Coinbase is a cryptocurrency exchange platform. Coinbase has $6$ Ethereum accounts and we treat them as one institutional account. We analyze the transaction history we collect and count the number of NW and NR, here NW is the amount of Ether transfer of Tx1 and NR is the amount of Ether transfer of Tx2 in each block. The average amount per block of NW and NR are $12.30$ and $34.76$. 

Under W1, M1’s cost of Coinbase is the following
$21000* NW + 21000 * NR$
The amortized cost of M1 is $21000$.

Under W1, M2’s cost of Coinbase is the following
$21000*L + 8332 * NW + 21000 * NR$
If $L = 1$, the amortized cost of M2 is $18135$, which saves $13.64\%$ than baseline, which is $21000$.

Under W1, M3’s cost of Coinbase is the following
$26512L + 1118 * NW+ 16036 * NR + NR*16 *(20+L)* 32*L +NR*(20+L)*222$
If $L = 1$, the amortized cost of M3 is $24085$, which costs $14.69\%$ more than baseline that is $21000$.

\begin{table*}[!htbp] %force in current page, disable float.
  \caption{Top-10 institutional senders}
  \label{tab:institutional-senders}
  \centering{\small
  \begin{tabularx}{0.97\textwidth}{ |X|l|l|l|l| }
    \hline 
  Sender & Amount percentage ($* 100\%$)& Value (Ether)  & Value percentage ($* 100\%$)\\ \hline
  $Ethermine (0x0xea67)$ & $4.81$ & $5306$ & $0.24$  \\ \hline
  $Coinbase 3 (0xddfabc)$ & $2.08$ & $18816$ & $0.87$   \\ \hline
  $Coinbase 4 (0x3cd751)$ & $2.08$ & $19127$ & $0.88$   \\ \hline
  $Coinbase 5 (0xb5d85c)$ & $2.05$ & $24248$ & $1.13$  \\ \hline
  $Coinbase 6 (0xeb2629)$ & $2.05$ & $20667$ & $0.96$   \\ \hline
  $F2Pool Old (0x829bd8)$ & $1.13$ & $2440$ & $0.11$   \\ \hline
  $Crypto.com (0x46340b)$ & $0.92$ & $5732$ & $0.27$   \\ \hline
  $FTX Exchange 2 (0xc098b2)$ & $0.81$ & $24320$ & $1.13$  \\ \hline
  $Hiveon: Spreader 2 (0x3c1618)$ & $0.78$ & $680$ & $0.03$   \\ \hline
  $Hiveon: Spreader (0xe7e6c8)$ & $0.76$ & $672$ & $0.03$   \\ \hline
  
  \end{tabularx}}
  \end{table*}


\subsection{The Case of Ethermine}

Ethermine is one of the top miners in Ethereum. The average amount per block of NW and NR are $4.65$ and $9.00$. 

Under W1, if $L = 1$, the amortized cost of M2 is $18222$, which saves $13.23\%$ than baseline that is $21000$. The amortized cost of M3 is $23059$, which costs $9.8\%$ more than baseline that is $21000$.

\subsection{The Case of Crypto.com}

Crypto.com is also a cryptocurrency exchange platform. The average amount per block of NW and NR are $1.49$ and $10.89$.

Under W1, if $L = 1$, the amortized cost of M2 is $21171$, which costs $0.82\%$ more than baseline that is $21000$. The amortized cost of M3 is $29941$, which costs $42.58\%$ more than baseline that is $21000$.

\section{Cost of mode M3 with blocks delay}

While the above delay-free method costs more than baseline, we introduce delay to update the digest and execute the Ether transferring. For each $K$ blocks, we upload a new digest and the state updating information on-chain, specifically the receiver's addresses and the transfer values. For every Ether transferring under W1 workloads, it takes $K - 1$ blocks delay at most. 

{\bf Under W1’ workload}: 

Under workload W1’, the cost is $21000L/K + NW [16 * (20 + 36) + 222] + (16 * 32 + 5000)L/K$ where $222$ is the cost of SHA3 Keccak-256 operation of two $32$ bytes digest, $16 * 32$ is the cost of uploading the new digest in the call data field and $5000$ is the cost of updating the digest for each $K$ block in the on-chain smart contract. Thus, the per-transfer cost is

$C_3 = 26512L/(NW*K) + 1118$

{\bf Under W1 workload}: Under workload W1, say $A_i$ has a initial balance in off-chain server and $A_i$ receive $V_i$ Ether in $L$ blocks, then $A_i$ sends Ether to another account, the cost is $21000L/K + NR [16 * (20 + 36 + 65) + 6600 + 7500] + NR*16 *(20+L/K)* 32*L/K +NR*(20+L/K)*222+ 5000L/K$ where $16 * (20 + 36 + 65)$ is the cost of uploading the receiver address, transfer value and sender’s signature, $6600$ is the cost of the verification process of the signature and $7500$ is the cost of an internal Ether transfer. $16 *(20+L/K)* 32*L/K$ is the cost of uploading the $20+L/K-level$ Merkle proof in each $K$ blocks. $(20+L/K)*222$ is the cost of $20+L/K$ SHA3 Keccak-256 operations to verify the digest. 

$C_3 = 26512L/K + 1118 * NW+ 16036 * NR + NR*16 *(20+L/K)* 32*L/K +NR*(20+L/K)*222$

\subsection{The Case of Coinbase}

We analyze the transaction history of Coinbase and count the number of NW and NR. If $K = 5$, the average amount per block of NW and NR are $59.64$ and $168.60$. 

Under W1, M1’s cost of Coinbase is the following
$21000* NW + 21000 * NR$
The amortized cost of M1 is $21000$.

Under W1, M2’s cost of Coinbase is the following
$21000*L/K + 8332 * NW + 21000 * NR$
If $L = 5$ and $K = 5$,  the amortized cost of M2 is 17781, which saves $15.32\%$ than baseline, which is $21000$.

Under W1, M3’s cost of Coinbase is the following
$26512L/K + 1118 * NW+ 16036 * NR + NR*16 *(20+L/K)* 32*L/K +NR*(20+L/K)*222$
If $L = 5$ and $K = 5$, the amortized cost of M3 is $23640$, which costs $12.57\%$ more than baseline that is $21000$.

\subsection{The Case of Ethermine}

Ethermine is one of the top miners in Ethereum. If $K = 5$, the average amount per block of NW and NR are $16.75$ and $32.46$. 

Under W1, if $L = 5$ and $K = 5$,  the amortized cost of M2 is $17114$, which saves $18.50\%$ than the baseline that is $21000$. The amortized cost of M3 is $21664$, which costs $3.16\%$ more than baseline that is $21000$.


\begin{wrapfigure}{r}{0.35\textwidth}
  \centering
  \includegraphics[width=0.324\textwidth]{figures/3workload-Delay.eps}
  \caption{Amortized Cost with blocks delay}
  \label{fig:workload-delay}
  \end{wrapfigure}

\subsection{The Case of Crypto.com}

Crypto.com is also a cryptocurrency exchange platform. If $K = 5$, the average amount per block of NW and NR are $6.70$ and $48.94$.

Under W1, if $L = 5$ and $K = 5$,  the amortized cost of M2 is $19851$, which saves $5.47\%$ than baseline that is $21000$. The amortized cost of M3 is $28274$, which costs $34.64\%$ more than baseline that is $21000$.

Figure~\ref{fig:workload-delay} shows the amortized cost per transfer with different delays. As the delay increases, the amortized cost gets lower. However, the amortized costs under these 3 workloads are still larger than the baseline. 

\section{Related Work}
{\bf Batching smart contract invocations}: iBatch~\cite{DBLP:conf/sigsoft/WangZLTCLC21} focuses on enabling secure batching of smart-contract invocations to optimize the base fee of a Ethereum transaction. iBatch uses a smart contract to dispatch each invocation, it doesn’t support Ether transfer between two Ethereum accounts and it requires the application smart contract rewrote to support iBatch. In iBatch protocol, all the states are stored on-chain, while OCIA stores the state off-chain to save the storage write cost. 

{\bf Layer-two}: Layer-two protocols~\cite{me:lightning,DBLP:journals/corr/MillerBKM17,DBLP:journals/corr/abs-1804-05141,DBLP:conf/ccs/DziembowskiFH18} builds an extension up on the blockchain. It executes the application logic off-chain, only storing the final result on-chain. It reduces the cost to two transactions, e.g. payment channel only needs open and close channel transactions. Layer-two protocol requires the participants no collusion, while OCIA doesn’t need any additional security assumption. 

{\bf Storing data off-chain}: GruB~\cite{DBLP:conf/middleware/LiTCYXX20} optimizes the cost in feeding external data to a blockchain. GruB stores data off-chain in write-intensive workloads and dynamically replicates the data on the blockchain. The saving of this dynamic replication is workload-specific in data feeding, while OCIA supports more general Ether transferring workloads. 

\section{Conclusion}

This paper presents OCIA, a scheme that stores the write-intensive account states off-chain to save the transaction cost. OCIA applies a trustless scheme to upload the states on-chain when it is read by on-chain transactions. The result shows the OCIA costs more than the baseline because of the overhead of verifying the off-chain states. 


==> text/abstract.tex <==
This paper presents OCIA, a blockchain cost optimization scheme for institutional accounts by leveraging batched processing and off-chain states. OCIA places the states of account balance to an untrusted off-chain server and dynamically uploads the states to the on-chain storage. OCIA supports secure Ether transfer without additional assumption. We study the cases of real-world institutional accounts, analyze their transaction traces, and estimate transaction costs. It shows that OCIA can save $18\%\sim{}47\%$ Gas cost per invocation under write-intensive workloads with a delay of $1.81\%\sim{}16.59\%$ blocks. 


==> text/wheels.tex <==
\section{learning}

\subsection{tables}

{\scriptsize \begin{verbatim} in beamer, see beamer_learn_slides. http://en.wikibooks.org/wiki/LaTeX/Tables#The_tabular.2A_environment_-_controlling_table_width
\end{verbatim}}

table with reference~\ref{tab:auth-attack}


\begin{table*}[!htbp] %force in current page, disable float.
\caption{Example of authorized searcher attack}
\label{tab:auth-attack}\centering{\small
\begin{tabularx}{0.5\textwidth}{ |X|c|c|c|c|c| }
  \hline
   & $p_0$ & $p_1$ & $p_2$ & $p_3$ & $p_4$ \\ \hline
  $r_a$ & $1$ & $0$ & $1$ & $0$ & $?$ \\ \hline
\end{tabularx}
}
\end{table*}

tabular (not table)

\begin{tabularx}{0.4\textwidth}{ |X|c|c|c| } %X is stretching to \textwidth, while c is to match with text width in cell.
  \hline
  label1                    & label2 & label3 & label4 \\ \hline
  \multirow{2}{*}{multi-row} 
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
  \multicolumn{2}{|l|}{multi-column}   & item3''  & item4''  \\  \hline
  \multirow{5}{*}{\begin{sideways}sideways\end{sideways}}
                             & item2  & item3  & item4  \\ \cline{2-4}
                             & \shortstack[l]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & \shortstack[r]{item2'\\item2''}  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \cline{2-4}
                             & item2'  & item3'  & item4'  \\ \hline
\end{tabularx}

\subsection{figures}
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\includegraphics[width=0.324\textwidth]{figures2/eff_rand_num_sample0.5.eps}
\caption{Wrapped figure}
\label{fig:perf}
\end{wrapfigure}

\ifdefined\TTUT
\begin{figure}[!ht]
\begin{center}
    \includegraphics[angle=90, width=0.45\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
\end{center}
%\vspace{-0.15in}
\caption{Easy figure}\label{fig:easy}
\vspace{-0.10in}\end{figure}

\begin{figure*}[!ht]
  \begin{center}
  %\goodgap
    \subfloat[Rotated]{%
      \includegraphics[angle=90, width=0.3\textwidth]{figures2/eff_rand_num_sample0.5.eps}%
      \label{exp:rand_num_1}%
    }%
    %\hspace{-0.2cm}%
    \subfloat[With more shared threads]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_num_sample2.eps}%
      \label{exp:rand_num_2}%
    }%
    \subfloat[With sample ratio]{%
      \includegraphics[width=0.3\textwidth]{figures2/eff_rand_sample_num10.eps}%
      \label{exp:rand_sample}%
    }%
  \end{center}%\vspace{-0.15in}
  \caption{Performance of optimization algorithm with random graph}\label{fig:complex}\vspace{-0.10in}
\end{figure*}
\fi

\subsection{algorithms}
\begin{algorithm}[h]
\caption{range-query(range $R$)}\small \label{alg:rangequery}
\begin{algorithmic}[1]
  \boldnext\State $\omega_R\leftarrow $ lowest-common-ancestor($R$) \Comment{comments: line number boldened}
  \State $\lambda\leftarrow $ DHT-lookup($f_{md}(\omega_R)$)
  \ForAll{$p \in P$} \Comment{comments: loop over all items}
    \State manipulate each term $p$
  \EndFor
  \If{$\lambda == NULL \And 1 \leq 0$}
      \State \Return lookup($R$.top\_left\_corner)
  \ElsIf{$R\subseteq{\lambda}$}
      \State \Return the keys of $\lambda$ that are in the range $R$
  \Else
      \State \Return recursive-forward($R$, $\omega_R$)
  \EndIf
\end{algorithmic}
\end{algorithm}

\subsection{equations}
\begin{eqnarray}
u &=& \sum_{l=0}^{n-1}{u_l} \mod{q} %\nonumber \\
=(\sum_{l=0}^{n-1}{ \sum_{j=0}^{c-1}{u_{l-j, j}} \mod{q}})\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{ \sum_{l=0}^{n-1}{ u_{l-j, j} } })\mod{q} %\nonumber \\
=(\sum_{j=0}^{c-1}{ \sum_{i=-j}^{n-1-j}{ u_{i, j} } })\mod{q} \nonumber \\
&=& (\sum_{j=0}^{c-1}{\sum_{i=0}^{n-1}{ u_{i, j} } }) mod q
= (\sum_{i=0}^{n-1}{ \sum_{j=0}^{c-1}{ u_{i, j} }\mod{q} })\mod{q} \nonumber \\
&=& \sum_{i=0}^{n-1}{ v_i }\mod{q} = \sum_{i=0}^{n-1}{ v_i } = v
\end{eqnarray}

With right brace
\begin{eqnarray}
\underline{\sigma}, \epsilon \rightarrow{}\underline{\beta_*}
\begin{cases}
\begin{rcases}
\begin{rcases}
& \sum_{\forall\beta_*>1}{(\beta_* - 1)} \\
& \sum_{\forall\beta_*<1}{(1 - \beta_*)} \\  
\end{rcases} \rightarrow{} \underline{X_1}\% \\
\sum_{\beta_*<1}{1} \rightarrow{} \underline{X_2}\%
\end{rcases}
\end{cases}
 \rightarrow{\beta}
\end{eqnarray}

\subsection{listing}
\lstset{language=SQL, style=Oracle, caption={Rewritten query against a single view table},label=sql:rewritten}
\lstset{frame=lrbt,xleftmargin=\fboxsep,xrightmargin=-\fboxsep} %with bounding box at l(eft)r(right)b(ottom)t(op)
%or you can replace it with "frame=single"
\begin{lstlisting}
  SELECT A, C FROM viewtable
  ORDER BY C LIMIT arg.k
\end{lstlisting}

\definecolor{mygreen}{rgb}{0,0.6,0}
\begin{figure}[h!]
%\begin{scriptsize}
%\begin{tabular}{cc}
%\begin{minipage}{.5\textwidth}
\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  %basicstyle=\footnotesize\ttfamily,        % the size of the fonts that are used for the code
  basicstyle=\scriptsize\ttfamily,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={(*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Java,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{black}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                  % show the filename of files included with \lstinputlisting; also try caption instead of title
  moredelim=[is][\bf]{*}{*},
}
\begin{lstlisting}
public void OnTouchEvent(MotionEvent e) {
Bitmap LoadPicture(String path) {
    ...
    *Bitmap bm = BitmapFactory.decodeFile(file)*;
    return bm;
}

void EditPicture(Bitmap bm) {
    //heavy computational picture editing
    int i = 10 (* $*$ *); //escape to plot * literatelly instead of bolden text
    bm.getPixels(pix, 0, mPhotoWidth, 0, 0, mPhotoWidth, mPhotoHeight);
    for(every pixel) {
      ...
    }  
    
    //embed location information into picture
    (* $*$*)Location loc = getLastKnownLocation(Provider)*;
    (* $*$*)double longitude = loc.getLongitude()*;
    (* $*$*)double latitude = loc.getLatitude()*;
    (* $*$*)EmbedLocation(bm, longitude, latitude);*
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
%\end{scriptsize}
\caption{Privacy-preserving Offloading Example}
\label{figure:MotivatingExample}
\end{figure}


\subsection{fbox}
\begin{center}
\fbox{This is a sample statement}
\end{center}

\begin{center}
\fbox{\parbox{0.90\linewidth}{
This is a long long long statement: 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
Blah blah blah blah 
}}
\end{center}



\subsection{misc}
\begin{itemize}
  \item cmark $\cmark$ and xmark $\xmark$
  \item bold math type $\boldsymbol{<v_0, k>}$
  \item use other than default font size: {``\fontsize{8.5}{9} this's in font size 8.5''}. (second param. should be 1.2$\times$ first param. which is font size
  \item show tilde in url, use \textasciitilde{} rather than \~{}
  \item strike out text, \sout{text/$12$ removed}
  \item color, {\color{red}red}{\color{green}green}
  \item[$\bullet$] big bullet on each item
  \item circled text \circled{2}
  \item A white number inside a black circle: \ballnumber{37}
  \item empty set (beautiful version) $\varnothing$ (needs ``\\usepackage\{amssymb\}''), which renames emptyset, $\emptyset$
  \item stackrel $\stackrel[c]{a}{=}$
\end{itemize}

citation for long breakable url~\cite{me:mssgx}

